Self-conditioning pre-trained language models

In this paper we aim to investigate the mechanisms that guide text generation with pre-trained Transformer-based Language Models (TLMs). Grounded on the Product of Experts formulation by Hinton (1999), we describe a generative mechanism that exploits expert units which naturally exist in TLMs. Such units are responsible for detecting concepts in the input and conditioning text generation on such concepts. We describe how to identify expert units and how to activate them during inference in order to induce any desired concept in the generated output. We find that the activation of a surprisingly small amount of units is sufficient to steer text generation (as little as 3 units in a model with 345M parameters). While the objective of this work is to learn more about how TLMs work, we show that our method is effective for conditioning without fine-tuning or using extra parameters, even on fine-grained homograph concepts. Additionally, we show that our method can be used to correct gender bias present in the output of TLMs and achieves gender parity for all evaluated contexts. We compare our method with FUDGE and PPLM-BoW, and show that our approach is able to achieve gender parity at a lower perplexity. The proposed method is accessible to a wide audience thanks to its simplicity and minimal compute needs. The findings in this paper are a step forward in understanding the generative mechanisms of TLMs.

==> preamble.tex <==

% if you need to pass options to natbib, use, e.g.:
%     \PassOptionsToPackage{numbers, compress}{natbib}
% before loading neurips_2020

% ready for submission
% \usepackage{neurips_2020}

% to compile a preprint version, e.g., for submission to arXiv, add add the
% [preprint] option:
%     \usepackage[preprint]{neurips_2020}

% to compile a camera-ready version, add the [final] option, e.g.:
     \usepackage[final]{neurips_2020}

% to avoid loading the natbib package, add option nonatbib:
%     \usepackage[nonatbib]{neurips_2020}

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{svg}

\title{Finding Experts in Transformer Models}

% The \author macro works with any number of authors. There are two commands
% used to separate the names and addresses of multiple authors: \And and \AND.
%
% Using \And between authors leaves it to LaTeX to determine where to break the
% lines. Using \AND forces a line break at that point. So, if LaTeX puts 3 of 4
% authors names on the first line, and the last on the second line, try using
% \AND instead of \And before the third author name.

\author{%
  Xavier Suau\\
  Apple\\
  \texttt{xsuaucuadros@apple.com} \\
  \And
  Luca Zappella \\
  Apple\\
  \texttt{lzappella@apple.com} \\
    \And
  Nicholas Apostoloff \\
  Apple\\
  \texttt{napostoloff@apple.com} \\
  % examples of more authors
  % \And
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
  % \AND
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
  % \And
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
  % \And
  % Coauthor \\
  % Affiliation \\
  % Address \\
  % \texttt{email} \\
}

==> sections/intro_ICML.tex <==
\section{Introduction }
\label{sec:introduction}

% Luca's proposal
Natural Language Processing (NLP) has evolved at a fast pace. For instance, language models \cite{Bengio:JMLR:2003} based on the Transformer \cite{Vaswani:NIPS:2017} architecture (\TM) achieve impressive performance in many tasks, including text generation \cite{Radford:ARXIV:2019,brown2020language}. Despite their success, the mechanisms that govern \TM generation remain unclear. Besides that, \TM have two important drawbacks:(1) conditioning these models to constrain the content of their generation requires either expensive re-training \cite{Keskar:Arxiv:2019} or the use of additional parameters \cite{Dathathri2020Plug,zhang2020side,Yang2021}; (2) \TM might inherit and perpetuate biases present in the training data, which can have a negative social impact \cite{sheng2019woman,AbubakarNature2021}, especially when \TM are deployed in commercial applications.

This paper aims to shine some light on the internal mechanism used by \TM to control text generation. We show that pre-trained \TM contain \emph{expert units} (neurons) that are responsible for detecting the presence of a specific concept within the initial context. We further observe that these expert units are responsible for steering the generation to be aligned with such concept. Throughout this paper we refer to \textit{concept} as an ``abstract idea''. A concept is anything that can be described with a set of examples that contain (positive examples) or do not contain (negative examples)  that concept. Concepts can be broad such as \textit{sport} or more precise one such as \textit{football}, \textit{world cup}, \textit{national football team}, \textit{player}, etc. In \secref\ref{sec:sentenceconcepts} we explain how concepts are formally represented.

In \secref\ref{sec:method} we show how these expert units can be found in a scalable manner for a variety of concepts, and then, how the identified experts can be used to induce the presence of a desired concept by activating its corresponding units \footnote{Link to the code will be made public upon acceptance.}. We observe that \TM require an extremely small amount of active experts to produce text with a specific concept (as little as 3 units in a model with 345M parameters), which support the hypothesis that \TM rely on those experts in order to generate sentences which are coherent with the context provided.

This finding has a natural application to self-conditioning in order to steer the generated output. In \secref\ref{sec:results_generation} we provide qualitative results on controlled generation with different concepts, including fine-grained homograph. 
In \secref\ref{sec:results_parity} we present an application of conditioning to the task of bias mitigation. We compare our method with two state of the art conditioning algorithms: \fudge \cite{Yang2021}, and PPLM \cite{Dathathri2020Plug} in its Bag-of-Words version (\pplm). While the aim of this work was to investigate how \TM work, the quality of the generated sentences is comparable with algorithms that are designed specifically for conditioning. In fact, we show that our method achieves \emph{generative parity} (\ie, the \oneTM generates sentences with equal probability of containing specific concepts) at lower perplexity, and with fewer instances of the specific concept keywords. This means that by using the experts a concept can be induced in a more complex and subtle way, than simply inducing the presence of a keyword. We observe that we can achieve parity by intervening on very few expert units (a median of 15 units, representing 0.0067\% of the model units analyzed). We further show that our conditioning is better correlated with the intrinsic bias of the model. Finally, in \secref\ref{sec:limitations} we discuss the limitations and potential improvements of our work.

NO REFERENCES TO SOTA AND CONCLUSIONS?

==> sections/intro_short_v3.tex <==
\section{Introduction }
\label{sec:introduction}

Natural Language Processing (NLP) has evolved at a fast pace. For instance, language models \cite{Bengio:JMLR:2003} based on the Transformer \cite{Vaswani:NIPS:2017} architecture (\TM) achieve impressive performance in many tasks, including text generation \cite{Radford:ARXIV:2019,brown2020language}. However, \TM have two drawbacks: (1) conditioning these models to constrain the content of their generation requires either expensive re-training \cite{Keskar:Arxiv:2019} or the use of additional parameters \cite{Dathathri2020Plug,zhang2020side,Yang2021}; (2) \TM might inherit and perpetuate biases present in the training data, which can have a negative social impact \cite{sheng2019woman,AbubakarNature2021}, especially when \TM are deployed in commercial applications.

In this paper, we show that pre-trained \TM already contain \emph{expert units} (neurons) that are responsible for inducing a specific concept in the generated text. Throughout this paper we refer to \textit{concept} as an ``abstract idea''. A concept is anything that can be described with a set of examples that contain (positive examples) or do not contain (negative examples)  that concept. Concepts can be broad such as \textit{sport} or more precise one such as \textit{football}, \textit{world cup}, \textit{national football team}, \textit{player}, etc. In \secref\ref{sec:sentenceconcepts} we explain how concepts are formally represented.

Previous work has already identified specialized units in pre-trained NLP models \cite{radford2017learning} as well as in the image domain \cite{Bau:CVPR:2017,Bau:ICLR:2019}. Our approach shows how these expert units can be found in a scalable manner for a variety of concepts, and subsequently be used to condition pre-trained \TM. We define as expert units those units that detect the presence of a concept in the \oneTM input with high accuracy. Interestingly, we observe that \TM require an extremely small amount of expert units to produce text with a specific concept  (as little as 3 units in a model with 345M parameters). This observation hints that a generative mechanism of \TM is based on very specific units acting as input detectors, and that the \TM use them as reliable sources of information to produce the output. In \secref\ref{sec:method} we propose an algorithm to exploit such generative mechanism by identifying expert units and applying a post-hoc intervention upon those units which increases the presence of a concept in the generated text without fine-tuning or additional parameters\footnote{Code will be released upon acceptance.}. 

% An interesting finding is that the number of expert units required for conditioning is extremely small compared to the size of \TM (less than 60 units in a model with 345M parameters).
% To the best of our knowledge, PPLM \cite{Dathathri2020Plug} in its Bag-of-Words version (\pplm) is the only work that achieves conditional generation without adding additional parameters. 
% In \secref\ref{sec:results_parity} we show that our method outperforms \pplm and improves over \fudge \cite{Yang2021} in several aspects.

% We propose a method to condition the generation of \TM without fine-tuning or using additional parameters and show that such conditioning can be used to study and mitigate biases. 
% We show that pre-trained \TM already contain \emph{expert units} that are responsible for inducing a specific \emph{concept} in the generated text. Previous work has already identified specialized units in pre-trained NLP models \cite{radford2017learning} as well as in the image domain \cite{Bau:CVPR:2017,Bau:ICLR:2019}.
% Our approach shows how these expert units can be found in a scalable manner for a variety of concepts, and used to condition pre-trained \TM.  To the best of our knowledge, PPLM \cite{Dathathri2020Plug} in its Bag-of-Words version (\pplm) is the only work that achieves conditional generation without adding additional parameters. In \secref\ref{sec:soa} we discuss how our approach compares with \pplm and other related works.

% We use the noun \emph{concept} as per its OxfordLanguages\footnote{https://languages.oup.com} definition: ``an abstract idea''. 


% In \secref\ref{sec:method} we propose an algorithm to identify \oneTM expert units  responsible for generating text that contains a specific concept. 
% We also propose a post-hoc intervention upon expert units that increases the presence of a concept in the generated text without requiring fine-tuning or additional parameters. 


In \secref\ref{sec:results_generation} we exploit the expert-based generative mechanism of \TM to condition on a variety of concepts (including fine-grained homograph concepts) and we provide qualitative generation results.
In \secref\ref{sec:results_parity} we show how gender bias is propagated in \TM generated text and that our technique can be used to mitigate it. \secref\ref{sec:results_parity} we compare with \fudge \cite{Yang2021} and PPLM \cite{Dathathri2020Plug} in its Bag-of-Words version (\pplm). To the best of our knowledge, \pplm and our method are the only works that achieve conditional generation without additional parameters. We show that our method achieves \emph{generative parity} (\ie,  the \oneTM generates sentences with equal probability of containing specific concepts) at lower perplexity and with fewer instances of the concept keywords. We further show that our conditioning is better correlated with the intrinsic bias of the model, and we observe that we can achieve parity by intervening on very few expert units (a median of 15 units, representing 0.0067\% of the model units analyzed). We further validate empirically our choice of expert units. Finally, in \secref\ref{sec:limitations} we discuss the limitations and potential improvements of our work.

% More precisely, we assess on how many expert units one must intervene upon to achieve \emph{generative parity} (\ie,  the \oneTM generates sentences with equal probability of containing specific concepts). Results show that our approach achieves generative parity by intervening on very few expert units (a median of 15 units, representing 0.0067\% of the model units analyzed), while still producing sentences with a median increase in perplexity smaller than 10\% with respect to the unconditional model. We compare our approach with \fudge and \pplm, showing that we achieve parity at lower perplexity. Finally, in \secref\ref{sec:limitations} we discuss the limitations and potential improvements of our work.

==> sections/introduction.tex <==

\section{Introduction }
\label{sec:introduction}

Natural Language Processing (NLP) has evolved at a fast pace during recent years. Large and powerful language models  \cite{Bengio:JMLR:2003} based on the Transformer architecture (\TM) \cite{Vaswani:NIPS:2017} achieve impressive performance in many tasks, including text generation \cite{Radford:ARXIV:2019,brown2020language}. However, such powerful models present several disadvantages: (i) they are difficult to train due to both the size of models and datasets, and the compute resources required\footnote{For example, \cite{Nvidia:GITHUB:2019} was trained on 512 GPUs}; (ii) \TM inherit and perpetuate biases that can have a negative social impact \cite{AbubakarNature2021} and (iii) conditioning these models to constrain their generation to specific topics (e.g., sport, economy, etc.), sentiments, tenses, etc.,
%(iii) conditioning these models on concepts 
requires re-training \cite{Keskar:Arxiv:2019} or using additional parameters \cite{Dathathri2020Plug,zhang2020side,zeldes2020technical}.
%, and being limited to very specific concepts. 

% Moreover, it is not fully understood why these models perform so well. Inspired by observations in neuroscience stating that the human brain is a network of hierarchically organized specialized modules \cite{Hill:2006}, and that neurons become more selective as humans learn \cite{Najafi:Neuron:2019}, we aim to find these specialized modules in \TM: the expert units. We hypothesize that \textit{the presence of expert units is related to the knowledge acquired by \TM and to their performance.}


%Natural Language Processing (NLP) has evolved at a fast pace during recent years. Large and powerful models based on the Transformer architecture \cite{Vaswani:NIPS:2017} can now be trained on large datasets, achieving impressive performance on many NLP tasks, such as GLUE \cite{Wang:ICLR:2019} or SQuAD \cite{Rajpurkar:EMNLP:2016,Rajpurkar:ACL:2018}. Large \TM can also be specifically trained as Language Models (LM) \cite{Bengio:JMLR:2003}, achieving impressive performance \cite{Radford:ARXIV:2019,brown2020language}. Training \TM is tedious due to both the size of models and datasets, and requires resources that are unavailable to many users. For example, in \cite{Nvidia:GITHUB:2019} the model was trained on 512 GPUs. A recent trend is to pre-train  these large models on diverse datasets and make them available to the community \cite{Howard:ACL:2018,Devlin:NAACL:2018,Lample:ARXIV:2019,Yang:NEURIPS:2019,liu:ARXIV:2019,Sanh:ARXIV:2019,Radford:ARXIV:2019,brown2020language}, so that end-users can leverage the powerful features learnt to solve downstream tasks.

%However, it is not fully understood why these models perform so well. Inspired by observations in neuroscience stating that the human brain is a network of hierarchically organized specialized modules \cite{Hill:2006}, and that neurons become more selective as humans learn \cite{Najafi:Neuron:2019}, we aim to find these specialized modules in \TM: the expert units. We hypothesize that \textit{the presence of expert units is related to the knowledge acquired by \TM and to their performance.}

It is not fully understood why these models perform so well. 
Previous work in interpretability of models in the image domain has shown that CNNs and GANs learn representations of specific objects at convolutional unit level \cite{Bau:CVPR:2017,Bau:ICLR:2019} and by unit combinations  \cite{Fong:CVPR:2018, kim2018interpretability}, even if those objects were never explicitly labeled during training. The intuition is that the model builds a hierarchy of concepts useful for decision making.
%The key idea behind these works is to consider CNN feature maps as segmentation masks, which allows quantifying the coherence with a densely labeled image by means of Intersection Over Union (IOU). 
Inspired by these works, given concept we aim to find specialized units in \TM that are responsible for producing sentences that contain such concept: the expert units. 
There are, however, fundamental differences in how we identify experts : %(i) In NLP, it is harder to  define a concept with a single sentence, thus we adopt a representation that uses positive and negative exemplars, similar to approaches in the image domain \cite{kim2018interpretability}.
(i) Compared to \cite{Bau:CVPR:2017,Bau:ICLR:2019}, we define a concept using positive as well as negative examples. In our work, positive examples are sentences that according to the annotation contain a desired concept, while negative examples are sentences in which the concept does not appear.
%thus we propose to represent concepts with sets of positive and negative sentences as explained in \secref\ref{sec:sentenceconcepts}. 
%A total of 1344 concepts are collected leveraging the OneSec dataset \cite{Scarlini:ACL:2019}. 
(ii) We consider the most basic units in \TM, the neurons, as expert unit candidates, while all the other works use convolutional units. (iii) We compute Average Precision $\ap$ (\ie area under the precision-recall curve) to quantify how well a unit is able to identify a concept, instead of using the Intersection over Union \cite{Bau:CVPR:2017,Bau:ICLR:2019, Fong:CVPR:2018} or an SVM classifier \cite{Fong:CVPR:2018, kim2018interpretability}. (iv) All previously mentioned works deal with the image domain where spatial resolution can be fixed, since sentences can be arbitrarily long, we max-pool the unit responses in time to be invariant to length. The proposed method to identify and rank experts is detailed in \secref\ref{sec:respo_units}.

% \begin{figure}[t]
% \begin{center}

% {\fontsize{8}{10} \selectfont
% \setlength{\tabcolsep}{1mm}
% \begin{tabular}{p{0.95\columnwidth}l}
% \toprule

% \textsf{
% \hspace{-0mm}{\color{red}[recompute]We study the presence of expert units in pre-trained Transformer Models (\TM), and how they can be used to control text generation with \oneTM based Language Models (LMs).
% We define expert units to be neurons that are able to detect a concept in the input context with a given average precision,} hence being able to correctly classify a future ball's passing or shooting angle. We find that many multi-category TMs are specifically trained to indicate the accuracy of a given concept when following the instructions of a pre-specified skill coach and/or observers. In this experiment we test this hypothesis, using TMs that specialize in the shooting skills of throwing and catching.}\\
% \bottomrule
% \end{tabular}
% }
%   \caption{Example of generated text by GPT2-L conditioned on the WordNet concept \href{\wordnet{football}}{football\%1:04:00}{\protect\footnoteref{footwordnet}} ~by intervening only its top-50 expert units (0.012\% of the 414720 units analyzed). The beginning of this paper's abstract is given as context {\color{gray}(gray)}. Experts are determined by the method detailed in \secref\ref{sec:respo_units} and the model is conditioned following \secref\ref{sec:self-conditioning}. The off-the-shelf model is conditioned without re-training, fine-tuning or using additional parameters. Note the strong presence of concept \href{\wordnet{football}}{football\%1:04:00} in the generated text, including words like `coach' or `shooting'.  Even more interesting is how the the term `TM' appears in a sporting sense, and how TMs `specialize', taking the  context  into account.\vspace{-2mm}
% } 
%   \label{tab:intro_sentence}
% \end{center}
% \vspace{-3mm}
% \end{figure}


%However, why these models perform so well remains only a partially answered question. Inspired by observations in neuroscience stating that the human brain is a network of hierarchically organized specialized modules \cite{Hill:2006} and that neurons become more selective as humans learn \cite{Najafi:Neuron:2019}, and by similar observations in image CNN/GAN \cite{Bau:CVPR:2017,Bau:ICLR:2019}, we hypothesize that \TM also work by creating specialized modules: the \textit{expert units}. In \secref\ref{sec:respo_units} we propose how to find expert units and we show that theind specialized modules in \TM, the \textit{expert units}, to gain an understanding of what \TM learn.

%We consider the most basic units in \TM, the neurons, as expert unit candidates. We design a method to identify and rank expert units in \TM by measuring their ability to disambiguate concepts. A concept is represented by a binary dataset consisting of sentences that contain (positive) or not (negative) the concept. 
%%This representation gives the flexibility to create many types of concepts: from abstract (\ie sentiment or verbal tense) to sentences containing a specific keyword. 
%A dataset with 1344 concepts is proposed in \secref\ref{sec:sentenceconcepts}, based on the OneSec dataset \cite{Scarlini:ACL:2019}.

%Previous work in image processing has shown that CNNs and GANs learn representations of specific objects at a filter level \cite{Bau:CVPR:2017,Bau:ICLR:2019} and by filter combinations  \cite{Fong:CVPR:2018}, even if those objects were never explicitly labeled during training. The key idea behind these works is to consider CNN feature maps as segmentation masks, which allows quantifying the coherence with a densely labeled image by means of intersection over union (IOU). These works have also inspired our research, however there are fundamental differences in our work: (1) in the NLP domain it is harder to  define a concept with a single sentence, thus we propose to represent concepts with binary datasets of sentences; (2) we consider a unit as a classifier able to disambiguate a concept, which allows computing AUPR (area under the precision-recall curve) to quantify coherence; (3) since sentences can be of arbitrary length, we propose to be invariant to length by maxpooling the unit responses in time. The proposed method to identify expert units is detailed in \secref\ref{sec:respo_units}.


%Interpretability of machine learning models has become extremely popular as deep neural networks (DNN) have become mainstream. Despite DNNs impressive results, interpreting what they learn and why decisions are made is still an open question. Such lack of interpretation is emphasized in Transformer-based Models (\TM)  due to their size, eg. \cite{Nvidia:GITHUB:2019} recently trained a model with 8.3B parameters; and due the data nature, consisting of sentences of arbitrary length. 

%Natural Language Processing (NLP) has undergone a revolution during recent years. Large and powerful models, most of them based on the Transformer architecture \cite{Vaswani:NIPS:2017}, can now be trained on huge amounts of data, achieving impressive performance on many NLP tasks. However, training such models is tedious and requires a lot of resources, most of the time unavailable to the majority of users. A recent trend is to pre-train versions of these large models on rich and diverse datasets and make them available to the community \cite{Howard:ACL:2018,Devlin:NAACL:2018,Radford:ARXIV:2019,Lample:ARXIV:2019,Yang:NEURIPS:2019,liu:ARXIV:2019,Sanh:ARXIV:2019}, so that end-users can solve downstream tasks leveraging the powerful features learnt by these pre-trained models. 

%In many cases, \TM are trained using simple techniques, such as \emph{predict the next token} as in \cite{Radford:ARXIV:2019} or \emph{predict the masked tokens} as in \cite{liu:ARXIV:2019}. 
%Recently, Transformer-based Language Models (LM) \cite{Radford:ARXIV:2019} have gained media attention given their ability to generate very realistic text passages, arising ethical issues such as automated fake news generation  \cite{Metz:NYT:2019}.
%Despite the rather simple training techniques, these models excel at NLP tasks.  We hypothesize that the \TM learn high level concepts to be able to achieve such results. Previous work in the image field \cite{Bau:CVPR:2017,Bau:ICLR:2019} has shown that CNN and GAN learn  representations of specific objects at a filter level, even if those objects where never explicitly labeled. A follow-up work \cite{Fong:CVPR:2018} shows that some objects are better represented by a combination of filters at layer level. Motivated by these works we propose a method to interpret \TM by quantifying their ability to disambiguate concepts. 
%We represent a concept with a binary dataset consisting of sentences that contain (positive) and do not contain (negative) the concept. This representation gives the flexibility to create many types of concepts: from abstract (\emph{ie.} sentiment, verbal tense) to sentences containing a specific keyword.
%A fundamental difference with \cite{Bau:CVPR:2017,Bau:ICLR:2019} is that in CNNs the intermediate feature maps can be directly compared with the input or the output, which allows quantifying the coherence of filters with the input and also their causality. In the NLP domain, it is much harder to measure  the \emph{amount of concept} in the input or output. For that reason, we propose an alternative way of measuring coherence with the input by defining concepts as binary datasets of sentences, and we  show that those units that are the best predictors for a concept are actually causal. 


% In \secref\ref{sec:concept_repr} we show that concepts with similar meaning are co-learnt by a certain number of experts. We define concept overlap to quantify co-learning, and we show its utility for concept explainability. 

The presence of experts is exploited in \secref\ref{sec:self-conditioning} to condition pre-trained \TM using its own knowledge (self-conditioning) to generate text that contains a specific concept (see \tabref\ref{tab:generated_openai} for examples). 
Our approach builds on the Product of Experts (PoE) formulation introduced by Hinton in \cite{Hinton:ICANN:1999}. Some previous works have adopted the PoE formulation, for example  \cite{Nguyen:CVPR:2017} applies it to image generative models by training an external conditional expert. In \cite{Dathathri2020Plug} the PoE formulation is applied to \TM, where an external attribute model is used to steer the internal latent variables of the \oneTM to maximize the presence of a concept. Although not optimizing PoE explicitly, \cite{zhang2020side,zeldes2020technical} also propose using an external model acting as conditional expert to achieve controllability.
% In addition to applying PoE to a new domain (NLP) and new architecture (Transformer), 
A notable difference with \cite{Nguyen:CVPR:2017} and \cite{Dathathri2020Plug,zhang2020side,zeldes2020technical} is that we consider that \textit{the conditional expert in PoE already exists in the pre-trained model}. We propose to find the top experts as explained in \secref\ref{sec:respo_units} and enforce the conditional PoE expert via a $do()$ operation, as detailed by \eq\eqref{eq:forcing} in \secref\ref{sec:respo_units}.
Our method neither requires computing gradients and updating the \TM internal variables at each decoding step as in \cite{Dathathri2020Plug}, nor training additional parameters as in  \cite{zhang2020side,zeldes2020technical}.

Results show that a small number of experts is required to induce a concept, supporting our hypothesis that \TM accumulate evidence of a concept in specific units, and that these are used for language generation. For example, only 60 units (0.015\% of the units analyzed) are required to condition GPT-Large \cite{Radford:ARXIV:2019} on the Wordnet\footnote{\label{footwordnet}We use the WordNet sense key notation \texttt{lemma\%A:BB:CC}, clickable as web links across the paper.} \cite{Princeton:WordNet:2020} concept \href{\wordnet{bird}}{bird\%1:05:00}. We also show that intervening on experts can adjust a \oneTM's output for concept parity, and we present results for the specific  topic of gender parity.
%Other works have tackled \oneTM conditioning \cite{Hu:ICML:2017,Romanov:NAACL:2019,Chen:NAACL:2019,Keskar:Arxiv:2019}, all based on learning disentangled concepts during training. 
To the best of our knowledge, our work is the first to condition an off-the-shelf pre-trained \TM without fine-tuning, re-training or using additional parameters.  Furthermore, our method is extremely simple to implement and requires minimal compute resources as discussed in \secref\ref{sec:limitations}.


% \todo{MAYBE REMOVE, DEPENDING ON WHETHER WE ADD GENERALIZATION RESULTS OR NOT} 
% In \secref\ref{sec:concept_richness} we explore the importance of expert units beyond generation, showing that it is strongly correlated ($\rr=0.833$) with the generalization power of \TM.
% % In \secref\ref{sec:concept_richness} we define a metric called \textit{concept expertise}, and we show that it is strongly correlated ($\rr=0.833$) with the generalization power of \TM. 
% As a measure for model generalization we use the average performance on diverse downstream tasks: all GLUE tasks + SQuAD v1.1/2.0. 
% We propose an empirical method to compute the expertise level that better represents generalization.
% %We propose an empirical method to compute the optimal expertise level that maximizes the correlation between generalization and expertise. 
% The obtained expertise ($\ap$ above 0.985) shows that generalization is related to the presence of extremely good and diverse experts. Our approach  enables ranking \TM by expertise, without fine-tuning on large suites of downstream tasks (current practice), mitigating the need for hyper-parameter search and the problem of downstream task bias \cite{Niven:ACL:2019}. 
% Moreover, the proposed concept dataset can be easily enriched and adapted for finer model comparison.




%The results show the importance of accumulating experts in language modeling. 

%Our conditioning method, besides being extremely simple to implement, evidences the following: (1) Language Model conditioning can be done without fine-tuning, re-training or using additional parameters, (2) \TM learn concepts localized in very specific experts event if the concepts were not labeled during training and (3) the shows in an extremely simple way. Our proposal avoids re-training or fine-tuning the model The positive results reinforce the importance of accumulating experts in \TM. 
%Furthermore, by assessing the average precision of the best predictors per concept, we can quantify the number of concepts missed by \TM. We show that concept richness is a reliable measure of the generalization of \TM. The classical approach to measure generalization of \TM is by fine-tuning on different downstream tasks, grouped in benchmarks such as  GLUE \cite{Wang:ICLR:2019} or SQuAD \cite{Rajpurkar:EMNLP:2016,Rajpurkar:ACL:2018}. \TM are then ranked according to the aggregated performance. However, this approach has some disadvantages: (1) the performance relies on the fine-tuning hyper-parameters, which may differ across models, (2) \TM sometimes rely on statistical cues to solve downstream tasks \cite{Niven:ACL:2019}, which may produce a biased model ranking (those models able to better exploit such cues will perform better). We prove that the proposed model ranking using concept richness strongly correlated with the ranking achieved on GLUE and SQuAD. Our ranking is only a function of the concepts considered (that can be easily scaled up) and the untouched pre-trained model.

% Comparison of \TM is usually done by evaluating on downstream task benchmarks, for example GLUE \cite{Wang:ICLR:2019} or SQuAD \cite{Rajpurkar:EMNLP:2016,Rajpurkar:ACL:2018}. But most \TM are designed as task-agnostic models, so evaluating them on specific downstream tasks can bias  the comparison.  Such intuition is supported by a recent study \cite{Niven:ACL:2019} that shows that task-specific test sets widely used in the community may result in strongly biased results. We propose an alternative approach to study the generalization of \TM by measuring their ability to capture concepts, without requiring any downstream task evaluation. We prove that the model ranking using our method is strongly correlated with the ranking achieved when fine-tuning the \TM for a set of downstream tasks.

%Previous work in the image field \cite{Bau:CVPR:2017,Bau:ICLR:2019} has shown that CNN and GAN learn disentangled representations of specific objects, even if they were not trained specifically in that sense. We adopt some ideas from \cite{Bau:CVPR:2017,Bau:ICLR:2019} and propose a method to interpret Language Models by quantifying their ability to disambiguate concepts. 


%Language Models are trained to solve an NLP task that consists in predicting the next token (or word) given some previous tokens, called context. The above mentioned pre-trained models are a common starting point, where typically a LM head is trained on top of the pre-trained model. LM have gained attention recently given their ability to generate very realistic text passages, arising ethical issues such as automated fake news generation or plagiarism \cite{Metz:NYT:2019}.

%Despite the rather simple training techniques, LM are able to generate high quality text passages understandable by a human reader. We hypothesize that the LM learn high level concepts to be able to produce such outputs. Previous work in the image field \cite{Bau:CVPR:2017,Bau:ICLR:2019} has shown that CNN and GAN learn disentangled representations of specific objects, even if they were not trained specifically in that sense. We adopt some ideas from \cite{Bau:CVPR:2017,Bau:ICLR:2019} and propose a method to interpret Language Models by quantifying their ability to disambiguate concepts. 

%However, 

%Pre-trained LM are commonly evaluated on a suite of downstream tasks (ie. GLUE Benchmark by \cite{Wang:ICLR:2019}). Such type evaluations makes the comparison of pre-trained models harder, since it is hard to distinguish whether the performance comes from the pre-trained model itself or from the from the extra layers fine-tuned for the specific tasks. Having a procedural way to compare pre-trained models will result in a more objective benchmarking.

%In \secref\ref{sec:sentenceconcepts} we design a dataset of concepts represented by sentences. In \secref\ref{sec:respo_units} we describe a method to identify which units in a LM are responsible of a concept. In \secref\ref{sec:concept_repr} we propose a novel way to embed concepts in a common feature space, regardless of the concept nature. In \secref\ref{sec:results} we provide experimental results supporting the proposed methods and hypothesis. Finally, in \secref\ref{sec:conclusions} we discuss the results and envisage future lines of work.

%Summarizing, the main contributions of this work are: 
%\begin{enumerate}
%
%\item A dataset of concepts represented by positive and negative sentences, see \secref\ref{sec:sentenceconcepts}. \vspace{-2mm}
%\item The definiton of experts 
%\item We propose to consider individual units in a \oneTM as binary classifiers for a specific concept. This enables ranking responsible units for each concept, and identifying which concepts are present in the \oneTM.\vspace{-2mm}
%\item We show that the top predictor units for a concept are causal, and propose a simple method to enforce the presence of concepts in the output of a Language Model.
%%\item A concept representation that allows for placing concepts in a common space regardless of their nature, which can be used for concept retrieval and visualization.\vspace{-2mm}
%\item  A framework to measure the generalization of \TM with respect to concepts, showing its effectiveness when compared to typical multitask benchmarks (GLUE and SQuAD) that require specific fine-tuning.\vspace{-2mm}
%\end{enumerate}



==> sections/introduction_short.tex <==
\section{Introduction }
\label{sec:introduction}

Natural Language Processing (NLP) has evolved at a fast pace during recent years. Large and powerful language models \cite{Bengio:JMLR:2003} based on the Transformer architecture (\TM) \cite{Vaswani:NIPS:2017} achieve impressive performance in many tasks, including text generation \cite{Radford:ARXIV:2019,brown2020language}. However, such powerful models present several disadvantages: (i) they are difficult to train due to both the size of models and datasets, and the compute resources required\footnote{For example, \cite{Nvidia:GITHUB:2019} was trained on 512 GPUs}; (ii) conditioning these models to constrain the content of their generation requires re-training \cite{Keskar:Arxiv:2019} (which as just mentioned before could be impractical) or using additional parameters \cite{Dathathri2020Plug,zhang2020side,zeldes2020technical}; (iii) \TM could inherit and perpetuate biases that can have a negative social impact \cite{AbubakarNature2021}; 

In this work we propose a technique that can be used to condition the text generation without the need to re-train or add more parameters to the initial model. Such conditioning can be used to better guide the generation, and to study and mitigate potential biases inherited from the training data.

Our proposal borrows from a body of research that studies the interpretability of DNNs in the image domain \cite{Bau:CVPR:2017,Bau:ICLR:2019,Fong:CVPR:2018, kim2018interpretability}. In these works it is shown that convolutional units within the intermediate layers of a neural networks could act as classifiers or detectors for what they call {\em semantic concepts} (e.g., ``house'', ``face'', etc.)~even if those concepts where never explicitly labelled. Furthermore, \cite{Bau:ICLR:2019} shows that the manipulation of the output of those units can be used to influence the generation in GANs in order to ensure that a desired concept appears in the produced image.

In the NLP domain, one might wish to condition a \oneTM to generate content related to a specific topic (e.g., economy, sport, etc.), or with a particular tense or sentiment. Inspired by these ideas, we propose to find specialized units in \TM that are responsible for producing sentences that contain a desired concept: the expert units (or simply the experts). However, the creation such a framework for the NLP domain requires fundamental changes with respect to the image domain: the way a concept is represented, the definition of a unit (since in \TM there are no convolutional layers), and the way experts are found. In our approach we represent a concept with a set of positive and negative examples, \secref\ref{sec:sentenceconcepts}. We propose that each single neuron can be an expert unit candidate, and we identify experts for a given concept by finding those whose Average Precision (\ap, \ie the area under the precision-recall curve) is the highest for that concept (\ie those units that can act as a good classifier about the presence of a concept in the input sentence), \secref\ref{sec:respo_units}. Such definition of expert units allows us proposing a  self-conditioning framework in the \TM context  by leveraging the Product of Experts (PoE) formulation introduced in \cite{Hinton:ICANN:1999}, \secref\ref{sec:self-conditioning}. Our proposal is compared with existing literature in \secref\ref{sec:soa}.

Results, in \secref\ref{sec:generation}, show that once we have found experts for a concept, the manipulation of a very small number of them (e.g, 0.015\% of all unites in GPT-Large \cite{Radford:ARXIV:2019}) is sufficient to induce such concept in the generated sentences. We call this manipulation an {\em intervention}. We also show that our intervention can be used to study and mitigate the presence of bias and achieve {\em concept parity}: the generated sentences have equal probability of containing a specific set of concepts. For example, in the context of gender bias, when the model is proposed a sentence that begins with ``the nurse said that'', XX\% of the times the generated sentence implies that the nurse is a female (and the opposite for ``the doctor said that''). Via intervention we can produce sentences that are roughly equal in the probability of the subject being a male or a female.

To the best of our knowledge, our work is the first to condition an off-the-shelf pre-trained \TM without fine-tuning, re-training or using additional parameters.  Furthermore, our method is extremely simple to implement and requires minimal compute resources as discussed in \secref\ref{sec:limitations}.


==> sections/introduction_short_v2.tex <==
\section{Introduction }
\label{sec:introduction}

Natural Language Processing (NLP) has evolved at a fast pace. Language models \cite{Bengio:JMLR:2003} based on the Transformer architecture (\TM) \cite{Vaswani:NIPS:2017} achieve impressive performance in many tasks, including text generation \cite{Radford:ARXIV:2019,brown2020language}. However, \TM present a couple of inconveniences: (1) conditioning these models to constrain the content of their generation requires expensive re-training \cite{Keskar:Arxiv:2019} or the use of additional parameters \cite{Dathathri2020Plug,zhang2020side,zeldes2020technical}; 
%(2) \TM inherit and perpetuate biases present in the training data corpus, and such bias is transferred to the unconditional text generation. Moreover, perpetuating bias has a negative social impact \cite{sheng2019woman,AbubakarNature2021} when \TM are included in commercial systems.
(2) \TM might inherit and perpetuate biases present in the training data corpus, which can have a negative social impact \cite{sheng2019woman,AbubakarNature2021}, especially when \TM are included in commercial systems.
We propose a method to condition the generation of \TM without using additional parameters nor retraining and we show that such conditioning can be used to study and mitigate biases.

Previous works have studied how to condition \TM on specific control variables \cite{Hu:ICML:2017,Chen:NAACL:2019,Romanov:NAACL:2019,Keskar:Arxiv:2019}. These methods propose  \emph{training} techniques to condition the output distribution of the \oneTM. However, few works have explored the conditioning of pre-trained \TM without modifying them \cite{Dathathri2020Plug,zhang2020side,zeldes2020technical}. The majority of these works leverage an external model that is used as a conditioning knob to steer the \TM output. To the best of our knowledge, PPLM \cite{Dathathri2020Plug} in its Bag-of-Words version (\pplm) is the only work that achieves conditional generation without adding additional parameters. Similarly to \pplm, we adopt the Product of Experts (PoE) formulation introduced by \cite{Hinton:ICANN:1999}. The main difference is that we consider that the expert conditional model \emph{already exists in the \oneTM} (instead of using an external model as in \pplm) and we propose a way to steer it. To that end, in \secref\ref{sec:respo_units} we show how to identify \oneTM units (neurons) that are responsible for generating text with a specific concept. This intuition is inspired  by a set of works that discover specialized units in image neural networks \cite{Bau:CVPR:2017,Bau:ICLR:2019,Fong:CVPR:2018, kim2018interpretability}. We call these units \emph{expert units}, and we propose in \secref\ref{sec:self-conditioning} a post-hoc intervention upon them that increases the presence of a concept in the generated text without requiring fine-tuning or additional parameters. We use a broad meaning of the word  \emph{concept}, which can encapsulate abstract topics such as sentiment, more precise ones like politics or sports, or even a specific word sense. In \secref\ref{sec:sentenceconcepts} we explain how concepts are formally represented.

As mentioned before, one important aspect of \TM is their inherited bias. We address this issue by building a set of experiments focused on gender bias. More precisely, we assess on how many expert units one must intervene upon to achieve \emph{generative parity} (\ie the \oneTM generates sentences with equal probability of containing specific concepts).
Results show that our approach achieves generative parity by intervening on very few expert units (0.048\% of the units analyzed for GPT2), while still producing meaningful sentences. %We compare with \pplm, which saturates before achieving parity.
%In contrast, \pplm achieves parity at the cost of the text perplexity.
In contrast, \pplm's output distribution collapses at the parity points, producing unintelligible sentences.

% We include a comparison of our proposal with \pplm in \secref\ref{sec:generation}.

% However, \TM inherit and perpetuate biases present in the training data corpus, and such bias is transferred to the unconditional text generation. Moreover, perpetuating bias has a negative social impact \cite{sheng2019woman,AbubakarNature2021} when \TM are included in commercial systems.

% In this work, we explore two aspects of \TM: (1) the presence of specialized (expert) units that are responsible of generating text in specific domains, and (2) how to leverage expert units to condition pre-trained \LM without fine-tuning or adding additional parameters. We show how our conditioning method is effective to condition \TM to generate text with gender parity.

Summarizing, the main novelties proposed in this work are:
\begin{itemize}
    \item A method to find expert units by ranking \oneTM neurons by their ability to induce a concept in the generated text.
    \item Leveraging expert units, we propose an intervention to condition text generation without fine-tuning or adding additional parameters (self-conditioning).
    \item We show that our self-conditioning method is effective to induce \TM to generate text with gender parity without compromising the text perplexity.
\end{itemize}

% The remainder of the paper is organized as follows. In \secref\ref{sec:respo_units} we define expert units and propose a method to identify them. The self-conditioning algorithm is presented in \secref\ref{sec:self-conditioning}. We review the literature and comment on similarities and differences with our method in \secref\ref{sec:soa}. In \secref\ref{sec:generation} we present the experimental results, which include a study on gender parity, a comparison with \pplm, and empirical proof supporting the choice of expert units. Finally, limitations of our method as well as compute requirements are outlined in \secref\ref{sec:limitations}.

% Several recent works address bias in Language Models in different ways: at word embedding level \cite{gonen2019lipstick}, in cross-lingual embeddings \cite{zhao-etal-2020-gender} or study and mitigate gender bias in the specific case of abusive language \cite{park-etal-2018-reducing} (among many others). 


% Natural Language Processing (NLP) has evolved at a fast pace during recent years. Large and powerful language models \cite{Bengio:JMLR:2003} based on the Transformer architecture (\TM) \cite{Vaswani:NIPS:2017} achieve impressive performance in many tasks, including text generation \cite{Radford:ARXIV:2019,brown2020language}. However, such powerful models present several disadvantages: (i) they are difficult to train due to the size of the models, the amount of data needed, and the compute resources required\footnote{For example, \cite{Nvidia:GITHUB:2019} was trained on 512 GPUs}; (ii) conditioning these models to constrain the content of their generation requires re-training \cite{Keskar:Arxiv:2019} (which as just mentioned before could be impractical) or using additional parameters \cite{Dathathri2020Plug,zhang2020side,zeldes2020technical}; (iii) \TM could inherit and perpetuate biases that can have a negative social impact \cite{AbubakarNature2021}.



% In this work we propose a technique that can be used to condition the text generation without the need to re-train or add more parameters to the initial model. Such conditioning can be used to better guide the generation, and to study and mitigate potential biases inherited from the training data.

% Our proposal borrows from a body of research that studies the interpretability of DNNs in the image domain \cite{Bau:CVPR:2017,Bau:ICLR:2019,Fong:CVPR:2018, kim2018interpretability}. In these works it is shown that convolutional units within the intermediate layers of a neural networks could act as classifiers or detectors for what they call {\em semantic concepts} (e.g., ``house'', ``face'', etc.)~even if those concepts where never explicitly labelled. Furthermore, \cite{Bau:ICLR:2019} shows that the manipulation of the output of those units can be used to influence the generation in GANs in order to ensure that a desired concept appears in the produced image.

% In the NLP domain, one might wish to condition a \oneTM to generate content related to a specific topic (e.g., economy, sport, etc.), or with a particular tense or sentiment. Inspired by these ideas, we propose to find specialized units in \TM that are responsible for producing sentences that contain a desired concept: the expert units (or simply the experts). However, the creation such a framework for the NLP domain requires fundamental changes with respect to the image domain: the way a concept is represented, the definition of a unit (since in \TM there are no convolutional layers), and the way experts are found. In our approach we represent a concept with a set of positive and negative examples, \secref\ref{sec:sentenceconcepts}. We propose that each single neuron can be an expert unit candidate, and we identify experts for a given concept by finding those whose Average Precision (\ap, \ie the area under the precision-recall curve) is the highest for that concept (\ie those units that can act as a good classifier about the presence of a concept in the input sentence), \secref\ref{sec:respo_units}. Such definition of expert units allows us proposing a  self-conditioning framework in the \TM context  by leveraging the Product of Experts (PoE) formulation introduced in \cite{Hinton:ICANN:1999}, \secref\ref{sec:self-conditioning}. Our proposal is compared with existing literature in \secref\ref{sec:soa}.

% Results, in \secref\ref{sec:generation}, show that once we have found experts for a concept, the manipulation of a very small number of them (e.g, 0.015\% of all unites in GPT-Large \cite{Radford:ARXIV:2019}) is sufficient to induce such concept in the generated sentences. We call this manipulation an {\em intervention}. We also show that our intervention can be used to study and mitigate the presence of bias and achieve {\em concept parity}: the generated sentences have equal probability of containing a specific set of concepts. For example, in the context of gender bias, when the model is proposed a sentence that begins with ``the nurse said that'', XX\% of the times the generated sentence implies that the nurse is a female (and the opposite for ``the doctor said that''). Via intervention we can produce sentences that are roughly equal in the probability of the subject being a male or a female.

% To the best of our knowledge, our work is the first to condition an off-the-shelf pre-trained \TM without fine-tuning, re-training or using additional parameters.  Furthermore, our method is extremely simple to implement and requires minimal compute resources as discussed in \secref\ref{sec:limitations}.


==> sections/method.tex <==

\section{Representing concepts with binary sentence datasets 
%\todo{Some notation changes, similar to previous version.}
}
\label{sec:sentenceconcepts}
Throughout this paper we refer to \textit{concept} as an ``abstract idea'' that can be described with a set of examples.
We extend \cite{kim2018interpretability} to the NLP domain by describing a concept $c$ with a dataset  $\{\bx_i^c, b_i^c\}_{i=1}^N$ of $\np$ positive sentences that contain $c$ (\ie, $b_i^c=1$) and $\nm$ negative sentences that do \emph{not} contain $c$ (\ie, $b_i^c=0$), with $N=\np+\nm$. Each sentence $\bx_i^c$ is padded to a length $T$.
%A similar approach is used in \cite{kim2018interpretability} in the image domain.
%We propose a data-driven approach to describe a concept $c$ by collecting a dataset $\{\bx_i^c, b_i^c\}$ with $\np$ positive sentences that contain the concept ($b_i^c=1$) and $\nm$ negative sentences that do \emph{not} contain concept ($b_i^c=0$). 
Such flexible definition allows diverse types of concepts to be represented. They can be broad such as \textit{sport} or more precise one such as \textit{football}, \textit{world cup}, \textit{national football team}, \textit{player}, etc. Our definition also allows representing abstract concepts (\eg, sentiment) or very concrete ones (\eg, bags-of-words).  

% We construct our concept dataset leveraging the OneSec dataset \cite{Scarlini:ACL:2019}, which contains sentences with one keyword annotated with a WordNet sense  \cite{Princeton:WordNet:2020}. This allows representing concepts as words with a specific meaning, \eg we can now use the concept \emph{note} as a reminder or \emph{note} as a tone of certain pitch. 

%Concepts can also be abstract, \eg positive sentences could contain positive sentiment or verbs in present tense to represent the \emph{sentiment} or \emph{present tense} concepts respectively.
In this work, we specifically consider  positive sentences that contain a keyword with a specific WordNet sense, whereas negative sentences do not contain such keyword. 
Our method is not limited by the choice of a specific dataset. 
We chose OneSec because it is composed of Wikipedia articles, a corpora that was not used for the training of the GPT2 model \cite{Radford:ARXIV:2019} used in our experiments. 

%Another advantage of OneSec is that it was built only using  Wikipedia articles. This is specially important when reporting results using the GPT2 model \cite{Radford:ARXIV:2019}, which was intentionally trained without Wikipedia text.

%In addition to the above categories, we have collected abstract concepts:
%\begin{itemize}
%\item \textbf{Sentiment}: Positive and negative sentences sampled from the Stanford Sentiment Treebank dataset \cite{Socher:EMNLP:2013} with a sentiment score threshold of 0.5.
%\item \textbf{SentEval probe tasks}: We also consider the binary tasks in the SentEval probe datasets \cite{Conneau:ELRA:2018}. More precisely, the concepts considered are: Past/Present tense, Bigram shift, Subject singular/plural, Object singular/plural, Sentence short/long, Tree deep/shallow.
%%\item \textbf{Question}: Questions as positive sentences, answers and plain sentences as negative set. FROM WHERE?
%\end{itemize}
% We compile 1344 concepts, refer to \appref\ref{app:concept_list} for the complete list of concepts and details on the annotations.
%plus 14 \textit{abstract} concepts. 
%The number of sentences collected is constrained by availability in the source dataset. 
We limit the data per concept to $100 \leq \np \leq 1000$ and $100 \leq \nm \leq 1000$, randomly sampling when more than 1000 sentences are available. We use $\nm > \np$ to account for the much larger variance of negatives with respect to positives examples. The choice of $\np, \nm$ is arbitrary, and it is usually a trade-off between the compute resources available and the quality of the concept representation needed. We leave as future work an analysis on dataset size. Refer to \appref\ref{app:concept_list} for the complete list of concepts mapped and details on the annotations.


\section{Expert Units}
\label{sec:respo_units}

%Let $\{\bx_i^c, b_i^c\}_{i=1}^N$ be a dataset composed of $N$ sentences $\bx_i^c$ padded to a length $T$, and binary labels $b_i^c$ that indicate whether a sentence contains a specific concept $c$ or not. 
In a typical \TM setting, a sentence $\bx_i^c$ is consumed, and each \oneTM layer produces an intermediate tensor of shape  ${D^{\ell}\times T}$, where $D^{\ell}$ is the number of hidden units in layer $\ell$. In order to be agnostic with respect to the sequence length, intermediate tensors are max-pooled (ignoring pad tokens) in the temporal dimension and concatenated, yielding a sentence representation $\bz^{c} \in \mathbb{R}^{M}$, where $M=\sum_{\ell=1}^L D^{\ell}$ is the total number of hidden units analyzed in layers $1\ldots L$. Details on the layers analyzed in \oneTM architectures are shown in \appref\ref{app:layers_schema}.
Let $\mathbf{Z}^c = [\bz^{c,1}, \cdots, \bz^{c,N}] \in \mathbb{R}^{M \times N}$ be the response matrix obtained for the $N$ sentences representing concept $c$, where each row $\mathbf{Z}_{m,:}^c \in \mathbb{R}^{N}$ contains the responses of unit $m$ to the sentences $\{\bx_i^c\}_{i=1}^N$ that define concept $c$. Similarly, $\bz^{c}_m \in \mathbb{R}$ is the individual response of unit $m$.
%Let $\mathbf{Z}^c = [\bz_{1}^{c}, \cdots, \bz_{N}^{c}] \in \mathbb{R}^{M \times N}$ be the response matrix obtained for concept $c$, where each row $\mathbf{Z}^c(m) \in \mathbb{R}^{N}$ contains the responses of unit $m$ to the sentences $\{\bx_i^c\}_{i=1}^N$ that define concept $c$.

We treat each unit in the \oneTM as a binary classifier for the task $\by^c = \{b_i^c\}_{i=1}^N$. Thus, we define the \textit{unit expertise} $\ap_m^c$ as the Average Precision (\ie area under the precision-recall curve) when using the unit's responses as predictions for $\by^c$: $\ap_m^c = \ap(\mathbf{Z}_{m,:}^c, \by^c) \in [0, 1]$. We hypothesize that, given the size of \oneTM-based LMs, certain units will act as good classifiers for specific concepts: \textit{the expert units}.


% $[u_i^{(\ell, 1)}, \cdots, u_i^{(\ell, D^{\ell})}]^\top \in\mathbb{R}^{D^{\ell}}$ per layer. For simplicity the $(\ell, j)$ indexing is replaced by $m=1..M$, with $M$ being the number of units analyzed in the model. In this work we analyze units in the \oneTM layers shown in \fig\ref{fig:transformer_schema}.

% For a specific unit $m$ in the model, we collect its response $\bu_m^c \in \mathbb{R}^{N}$ to all the sentences  $\{\bx_i^c\}_{i=1}^N$ that define a concept $c$, and we treat the unit as a binary classifier for such dataset with groundtruth $\by^c = \{b_i^c\}_{i=1}^N$. Then, we define the \textit{unit expertise} $\ap_m^c = \ap(\bu_m^c, \by^c) \in [0, 1]$ as the average precision ($\ap$) when using the unit's responses as predictions for $\by^c$.

% Let $\bx_i = [\bx_{i, 1}, \cdots, \bx_{i, T}]\in \mathbb{R}^{D\times T}$ be a sentence composed of an arbitrary number $T$ of tokens $\bx_{i,t}\in\mathbb{R}^D$, with $D$ being the dimensionality of the token embedding. A layer $\ell$ of a \oneTM produces an intermediate representation $\bz_{i}^{\ell} = [\bz_{i, 1}^{\ell}, \cdots, \bz_{i, T}^{\ell}] \in \mathbb{R}^{D^{\ell}\times T}$, where typically $D^{\ell}$ is a multiple of $D$. Let $[u_i^{(\ell, 1)}, \cdots, u_i^{(\ell, D^{\ell})}]^\top \in\mathbb{R}^{D^{\ell}}$ be the intermediate representation max-pooled in the temporal dimension, where each element $u_{i}^{(\ell, j)}\in\mathbb{R}$ is the response of unit $j$ in layer $\ell$ to sentence $i$. 
% % response of the \emph{sub-network} $\bm{\theta}^{<(\ell,j)}$ prior to the unit, which uses a fraction of the total network parameters $\bm{\theta}$.
% %We analyze the units produced by the fully-connected layers in the Transformer blocks, as depicted in \fig\ref{fig:transformer_schema}.
% For simplicity the $(\ell, j)$ indexing is replaced by $m=1..M$, with $M$ being the total number of units in the model. The layers analyzed in \TM are shown in \fig\ref{fig:transformer_schema}. Let $\bu_c^m \in \mathbb{R}^{N_c}$ (where $N_c=\np+\nm$) be the pooled response of unit $m$ 
% to the sentences that represent concept $c$, and let $\by_c \in \mathbb{Z}_2^{N_c}$ be the binary labels for such sentences.  We treat a unit as a binary classifier for the input sentences, and consider the whole network as a collection of binary classifiers. By using $\bu_c^m \in \mathbb{R}^{N_c}$ as prediction scores for $\by_c$, we can compute the \emph{unit expertise} $\ap_c^m = \ap(\bu_c^m, \by_c) \in [0, 1]$ per unit $m$ and per concept $c$. We expect that, given the large search space, certain classifiers will perform well on specific concepts: the expert units.


In order to control the generation of \TM, we define the intervention on $k$ expert units as a $do(c,k)$ operation \cite{Pearl:Causality} on the model responses at inference time. Let $\mathcal{Q}_k$ be the indices of the top-$k$ units sorted by $\ap_m^c$, then the operation in \eq\eqref{eq:forcing} manipulates the responses $\bz^c(k)$ of the top-$k$ units by setting them to their expected value for concept $c$:
\begin{equation}
\small
\label{eq:forcing}
    do(c, k): \{\bz_{m}^c := E_{\bx^c}\big[\bz_{m}^c \,|\, \by^c = 1\big]\; \forall m \in \mathcal{Q}_k \}.
\end{equation}
Note that the expectation in \eq\eqref{eq:forcing} can be approximated as $E_{\bx^c}\big[\bz_m^c \,|\, \by^c = 1\big] \approx \nicefrac{(\by^c)^\top\mathbf{Z}_{m,:}^c }{\| \by_c\|_1}$. See \appref\ref{app:code} for a Pytorch \cite{pytorch2019} code example implementing \eq\eqref{eq:forcing}.





==> sections/method_v2.tex <==


\section{Self-conditioning}
\label{sec:method}
\subsection{Intervention on expert units}
\label{sec:respo_units}

We consider a neuron to be an expert unit for a given concept $c$ if its output can be used as a predictor for the presence of that concept. Formally, let $\bz_m^c = \{z^c_{m,i}\}_{i=1}^N$ be the outputs of neuron $m$ to sentences $\{\bx_i^c\}$. We treat $\bz_m^c$ as prediction scores for the task $\by^c = \{b_i^c\}_{i=1}^N$. Thus, we measure the \textit{expertise} of a unit $m$ for the task $\by^c$ ($\ap_m^c$) with its the Average Precision (\ie, area under the precision-recall curve), so that $\ap_m^c = \text{AP}(\bz_m^c, \by^c) \in [0, 1]$.  For each concept $c$ we measure the $\ap_m^c$ for all units and layers and rank them from the highest to the lowest level of expertise. Note that, to be agnostic with respect to the sequence length, the output of each layer is max-pooled  across the temporal dimension (ignoring pad tokens).

In order to induce the presence of a concept $c$ during text generation, we manipulate the responses of the top experts, irrespective of their input, to be equal to their typical values measured when $c$ is present. Borrowing from the causality literature \cite{Pearl:Causality}, we define the intervention on $k$ expert units as a $do(c,k)$ operation on the model responses at inference time. Let $\mathcal{Q}_k$ be the indices of the top-$k$ experts, then the operation in \eq\eqref{eq:forcing} manipulates the responses of the top-$k$ experts by setting them to their expected value for concept $c$:
\begin{equation}
\small
\label{eq:forcing}
    do(c, k): \{\bz_{m}^c := E_{\bx^c}\big[\bz_{m}^c \,|\, \by^c = 1\big]\; \forall m \in \mathcal{Q}_k \}.
\end{equation}
Note that the expectation in \eq\eqref{eq:forcing} can be approximated as $E_{\bx^c}\big[\bz_m^c \,|\, \by^c = 1\big] \approx \sum_{i=1}^{\np} z_{m,i}^c / \np$ (ignoring negative examples). See \appref\ref{app:code} for a PyTorch \cite{pytorch2019} code example that implements  \eq\eqref{eq:forcing}.


==> sections/self_conditioning.tex <==

\subsection{Self-conditioning pre-trained \TM
%\todo{Very similar to previous version, only included notation from section \ref{sec:respo_units}}
}
\label{sec:self-conditioning}
Language models are generative models that can generate text consistent with linguistic rules. More formally, autoregressive language models maximize the probability of a sentence $\bx$ as $p(\bx) = p(\bx_1,\ldots,\bx_{T}) = \prod_{t=1}^T p(\bx_t | \bx_{<t})$ \cite{Bengio:JMLR:2003}.
A conditional generative model maximizes the joint distribution $p(\bx, y)=p(y|\bx)p(\bx)$, where $\bx$ is the generated sentence and $y$ is a latent conditional variable (\ie, a concept in $\bx$). As proposed by \citet{Hinton:ICANN:1999}, this equation can be interpreted as a \textit{Product of Experts}. The same interpretation was adopted in \cite{Dathathri2020Plug,Yang2021} for conditioned text generation, where $p(y|\bx)$ is the expert model that determines the condition for generation, while $p(\bx)$ is the expert that ensures that the generated sequence lies within the manifold of sentence distributions.
%In \cite{Nguyen:CVPR:2017} a general formulation for conditioned generative models is proposed, stating that the joint sampling probability $p(\bx, y) = p(\bx)p(y|\bx)$ of $x$ and a condition $y$ is the product of the probabilities given by two experts: a $p(y|\bx)$ expert that determines the condition for generation, and a $p(\bx)$ expert ensuring that the generated sequence is within the manifold of sentence distributions. 
In conditioned generation, rather than jointly sampling $\bx$ and $y$, we define the condition $y=c$ before sampling $\bx$, thus 
\begin{equation}
\label{eq:conditioned_gen}
p(\bx|y=c) \propto p(y=c|\bx)p(\bx).
\end{equation}
Unlike \citet{Dathathri2020Plug} and \citet{Yang2021} that model $p(y=c|\bx)$ with an external network, we hypothesize that \textit{the condition expert $p(y=c|\bx)$ already exists \textit{within} the same model}, and that the model is able to maximize $p(\bx|y=c)$ by exploiting its internal condition expert.
This means that we condition the model using its own knowledge (self-conditioning), without the use of any external model or auxiliary training variables, and without fine-tuning.  
%In \cite{Nguyen:CVPR:2017} the authors propose to model $p(y=c|\bx)$ with an external network. 
%Contrarily to \cite{Nguyen:CVPR:2017}, we hypothesize that the condition expert $p(y=c|\bx)$ already exists \textit{within} the same model, and that the model is able to produce $p(\bx|y=c)$ by trusting its internal condition expert. 
%Such intuition is based on the fact that \TM are extremely large in size, having extra degrees of freedom to accommodate many condition experts. 
%This intuition is connected to findings in neuroscience \cite{Najafi:Neuron:2019} that show that the human brain increasingly relies on selective groups of neurons as it learns.
% If we can identify selective neurons that contribute to the condition expert $p(y=c|\bx)$, we can control the ``amount'' of concept $c$ in the generated sentences. 
%Of course, the quality of the experts will dictate how well the concept can the controlled.

The quality of the conditional expert model will dictate the extent to which a concept can be controlled during generation.
On the other hand, a good $p(\bx)$ is also required to ensure that the generated text stays within the language manifold; failing to do so would lead to sentences that maximize  $p(\bx|y=c)$ but are not linguistically correct. 

%First, a p(y|\bx) expert determines a condition for image generation (e.g. images have to be clas- sified as “cardoon”). Also, in a high-dimensional image space, a good p(\bx) expert is needed to ensure the search stays in the manifold of image distribution that we try to model (e.g. images of faces [6, 63], shoes [67] or nat- ural images [37]), otherwise we might encounter “fool- ing” examples that are unrecognizable but have high p(y|\bx) [38, 51]. 

In order to maximize \eq\eqref{eq:conditioned_gen} one can maximize $p(y=c|\bx)$ while keeping $p(\bx)$ unchanged. This is the case for pre-trained models, since we cannot improve $p(\bx)$ without re-training or fine-tuning the model. We propose to maximize $p(y=c|\bx)$ by increasing the number of experts $k$ when applying the $do(c,k)$ intervention, \eq~\eqref{eq:forcing}. Although such intervention modifies the model behavior, $p(\bx)$ should be minimally affected, since $k << M$ ($M$ being the total number of units available). Larger values of $k$ will eventually degrade $p(\bx)$ over $p(y=c|\bx)$ and the conditioned generative probability $p(\bx|y=c)$ will collapse. %Results in Fig.~\ref{fig:perplexity} support these claims.
 
% As explained in \secref\ref{sec:respo_units}, $\ap_c^m$ explains how well unit $m$ is able to classify concept $c$. We consider those units with high $\ap_c^m$ as internal condition experts for concept $c$, each accumulating evidence in $p(y=c|\bx)$.
%
%To control $p(y=c|\bx)$ we force the top-K experts to be active.
% to their median active value when concept $c$ is present in the input. 
%More formally, the forcing value for expert $m$ is $\tilde{u}_c^m = \text{median}(\bu_c^m|_+)$ where $\bu_c^m|_+ \in \mathbb{R}^{\np}$ are the responses to the set of positive sentences for $c$. 
%The larger K, the more concept $c$ will be present in the output, provided that the expert has learnt the concept. Too large K will result in illegible sentences, since $p(y=c|\bx)$ will dominate $p(\bx)$ in \eq\eqref{eq:conditioned_gen}.


%The proposed forcing strategy is inspired by  \cite{Bau:ICLR:2019}, where the authors use the mean filter response conditioned to the presence of some object in an image generated by a GAN. We adapt their approach to the LM case: 
Autoregressive language models generate text via sequential decoding, which ties the presence of a concept in the input and the output of a \oneTM. 
% Indeed, the presence of a concept in the context $\bx_{<t}$ will translate to the presence of the concept in the generated text $\bx_{t}$. 
For example, words related to \textit{football} are more likely when the input is about \textit{football}. We apply the $do(c,k)$ operation in \eq~\eqref{eq:forcing} to artificially simulate the presence of a concept in the input. By setting the responses of expert units to the values they typically have when the concept is present, we effectively induce the model to behave as if the concept is present in the input.

% Results in \secref\ref{sec:units_choice} support the choice of the top-$k$ experts by $\ap_m^c$ as a reasonable strategy to condition generation. We specifically show that the top-$k$ group of experts achieves a much higher concept probability than other groupings, which is very important given the extremely large search space (\eg  $1.28\times 10^{136}$ possible groups of $k=30$ for GPT2-L).

%Note that the total number of possible groups is $\binom{M}{k}$, which for GPT2-L results in an intractable number of $1.28\times 10^{136}$ possible groups ($k=30$). 
%we cannot quantify the presence of $c$, however the output and the input of LMs are tightly related given the sequential decoding, which allows the forcing value to be computed as the mean active value when concept $c$ is present in the input (\eq~\eqref{eq:forcing}); 
%(2) our expert identification strategy is by $\ap$ given a binary dataset, while  \cite{Bau:ICLR:2019} considers CNN filter responses as segmentation masks to compute IOU with a labeled image.
The results in \secref\ref{sec:generation} confirm our hypothesis that the conditional expert exists within the model, and that the model leverages it to self-condition generation. Specific results in \secref\ref{sec:units_choice} also validate our ranking of expert units.
% We would like to remark that the proposed technique allows self-conditioning pre-trained LM. That is, conditioning without the use of any external model or auxiliary training variables, and without the need to re-train or fine-tune the model. 
% To the best of the authors knowledge, this is the first work to apply self-conditioned text generation on off-the-shelf pre-trained \oneTM. 

% Further exploration in the generative field, although extremely interesting, is out of scope for this work.

%Note that the successful results in \secref\ref{sec:generation} empirically reinforce our proposal of identifying responsible units using $\ap_c^m$, and shows that responsible units are also causal in the framework of Language Models.

%\begin{algorithm}
%\caption{Self-conditioned text generation for concept $c$}\label{alg:cap}
%\label{alg:selfcondition}
%\begin{algorithmic}
%\Require Model responses $\mathbf{Z}^c$ to data $\{\bx_i^c\}$, labels $\by^c$, %units conditioned $k$, units analyzed $M$
%\vspace{1mm}
%\Procedure{FindExperts}{$\mathbf{Z}^c, \by^c, k$}
%\State $\ap_m^c \gets \text{AP}(\mathbf{Z}_{m,:}^c, \by^c)\quad\forall m\in M$ %\Comment{\secref\ref{sec:respo_units}}
%\State $\mathcal{Q}_M \gets \texttt{argsort(}\ap_m^c\texttt{)}$
%\State \textbf{return} $\mathcal{Q}_M$
%\EndProcedure
%\vspace{1mm}
%\Procedure{SelfConditionedGen}{$\mathcal{Q}_M, k$}
%\State $\mathcal{Q}_k \gets \mathcal{Q}_M\texttt{[:-k]}$
%\State $\bz_m^c \gets \frac{(\by^c)^\top\mathbf{Z}_{m,:}^c}{\| \by_c\|_1}\quad %\forall m \in \mathcal{Q}_k$  \Comment{\eq\eqref{eq:forcing}}
%\State GenerateSentence()
%% \For{desired num tokens}
% \State Generate token
%% \EndFor
%\EndProcedure
%\end{algorithmic}
%\end{algorithm}

% \begin{algorithm}
% \caption{Self-conditioned text generation for concept $c$}\label{alg:cap}
% \label{alg:selfcondition}
% \begin{algorithmic}[1]
% % \Require Model responses $\bz_{m, i}^c$ to data $\{\bx_i^c\}$, labels $\by^c$, units conditioned $k$, units analyzed $M$.
% \vspace{-1mm}
% \Procedure{FindExperts}{$\bz_{m,i}^c, \by^c, k$}
% \State $\ap_m^c \gets \text{AP}(\bz_m^c, \by^c)\quad\forall m\in M$ \Comment{\secref\ref{sec:respo_units}}
% \State $\mathcal{Q}_M \gets \texttt{argsort(}\ap_m^c\texttt{)}$
% \State \textbf{return} $\mathcal{Q}_M$
% \EndProcedure
% \vspace{1mm}
% \Procedure{SelfCondGen}{$\mathcal{Q}_M, \bz_{m,i}^c, k$}
% \State $\mathcal{Q}_k \gets \mathcal{Q}_M\texttt{[:-k]}$
% \State $\bz_m^c \gets \sum_{i=1}^{\np} \bz_{m,i}^c / \np\; \forall m \in \mathcal{Q}_k$  \Comment{\eq\eqref{eq:forcing}}
% \State GenerateSentence()
% % \For{desired num tokens}
% % \State Generate token
% % \EndFor
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

